Reliability Evaluation of Individual Predictions: A Data-centric Approach

Machine learning models only provide probabilistic guarantees on the expected loss of random samples from the distribution represented by their training data. As a result, a model with high accuracy, may or may not be reliable for predicting an individual query point. To address this issue, XAI aims to provide explanations of individual predictions, while approaches such as conformal predictions, probabilistic predictions, and prediction intervals count on the model's certainty in its prediction to identify unreliable cases. Conversely, instead of relying on the model itself, we look for insights in the training data. That is, following the fact a model's performance is limited to the data it has been trained on, we ask "is a model trained on a given data set, fit for making a specific prediction?". Specifically, we argue that a model's prediction is not reliable if (i) there were not enough similar instances in the training set to the query point, and (ii) if there is a high fluctuation (uncertainty) in the vicinity of the query point in the training set. Using these two observations, we propose data-centric reliability measures for individual predictions and develop novel algorithms for efficient and effective computation of the reliability measures during inference time. The proposed algorithms learn the necessary components of the measures from the data itself and are sublinear, which makes them scalable to very large and multi-dimensional settings. Furthermore, an estimator is designed to enable no-data access during the inference time. We conduct extensive experiments using multiple real and synthetic data sets and different tasks, which reflect a consistent correlation between distrust values and model performance.

==> user_study.tex <==
\vspace{-5mm}
\color{orange}
\section{Study of User Preferences}
\vspace{-2mm}
We ran a study to evaluate the user preferences and our design choices for Trustworthy AI. 
Sending anonymous voluntary survey requests to the graduate students of the computer science department at the University of Illinois Chicago with fundamental knowledge of machine learning and data science, we obtained responses from {\bf 51 participants}. 
The participation was voluntary and completely anonymous with no personal information collected.

\stitle{Q1. Reliability Warnings \textcolor{orange}{vs.} Explainability}
As explained in \S~\ref{sec:related}, there has been extensive research on explaining the outputs of ML models. Such explanations by approaches, including LIME, SHAP, and QII, aim to justify the model outputs. Conversely, our proposal raises a warning signal when the model outputs are not reliable based on the dataset they have been trained on. In our first question, we surveyed the participants about which of these two they would find more helpful.
In particular, we asked the question ``Which one of the following would find more valuable for critical decision making: (i) Reliability warnings that would raise a flag when an output is not trustworthy. (ii) Approaches that provide an explanation of the model output, irrespective of how reliable it is.''.
While only one of the participants believed neither of the two are needed, 17.6\% preferred only the approaches that explain model outputs, and 21.6\% of the participants preferred only reliability warnings.
Still, aligned with our explanation in the introduction, the majority of the participants (58.8\%) agreed that {\bf both approaches should co-exist alongside each other}.


% In the first question, we asked the participants if, for critical decision-making, reliability warnings that indicate untrustworthy outputs are more valuable or approaches that explain model outputs, regardless of their reliability. 21.6\% of the participants preferred reliability warnings while 17.6\% preferred the approaches that explain model outputs. 58.8\% of the participants mentioned that both alternatives should co-exist alongside each other while 2\% claimed that neither is required and the model output is enough.

\stitle{Q2. Model dependent/independent Metrics}
As discussed in \S~\ref{sec:related}, the existing research on the reliability of predictions includes metrics such as Conformal Prediction, Prediction Intervals, and Prediction Probabilities which aim to estimate the uncertainty from the models themselves. On the other hand, our proposed metrics are model-independent and capture the unreliability based on the dataset. 
In our second question, we asked the participants about their preference for model-dependent and model-independent metrics to quantify the reliability of predictions. 5.9\% favored model-dependent measures such as conformal predictions and predictive probabilities that use the model itself to evaluate how trustworthy its output is are reliable enough for critical decision-making. Still, aligned with our proposal, 94.1\% of the participants believed that {\bf a model itself may not be enough for identifying its own flaws, and hence, model-independent metrics are needed to evaluate how reliable a model output is}. 

\stitle{Q3. Model Confidence Pitfall}
ML provides guarantees under the i.i.d assumption where training data used to build a model are independently and randomly sampled from the original underlying distribution. This assumption may not hold in real-world scenarios. Therefore, a model, while confident about its prediction according to model-dependent metrics, may not have observed sufficient training data from relevant regions. 
In our third question, we presented a similar scenario to the participants and asked them to declare their level of trust in the model's prediction. More specifically, we asked them to ``Rate their trust in the model's prediction on a scale of 1 (least) to 5 (highest), given a scenario where a model is 99\% confident in its prediction but lacks sufficient training data from the relevant region''. Results are presented in Figure \ref{fig:user_rating}. Around 61\% of the participants responded that {\bf they had little trust in the model's decision in the depicted scenario} which verifies our choice of including a lack of representation component in designing a reliability measure.
\vspace{-10mm}
\begin{figure}[H]
    \centering
    \includegraphics[width=.33\textwidth]{figs/user_rating.pdf}
    \vspace{-4mm}\caption{participants' level of trust in the model's prediction regarding Q3 of the user study.}
    \label{fig:user_rating}
    \vspace{-8mm}
\end{figure}

\stitle{Q4. Interpretability: Aggregated Reliability Score \textcolor{orange}{vs.} Multiple Scores}\marginpar{R1O3}
As explained in \S~\ref{sec:measures}, there are multiple factors associated with the unreliability of each prediction. Therefore, it is very important how to deliver the concluding message to the users.  
In our fourth question, we surveyed the users' preferences on the presentation and interpretability of the \ru measures.
More specifically, we asked the participants about their preference for assessing the reliability of an ML model's output as a decision-maker. 51\% of the participants responded that they preferred having multiple scores, each associated with a specific source of unreliability while the remaining 49\% favored a single unreliability score that combines various factors with explanations for a high score.
This motivates the need to {\bf provide the \ru value break-downs and the scores on each components} alongside the \ru scores, similar to Figure~\ref{fig:high_distrust_mock_interface}. 
% In line with the collected responses, {\bf we report the aggregated scores along with the contribution of each source of unreliability and an explanation of the reason behind the score}. \nima{Abol, please check the message.}

\stitle{Q5. Binary \textcolor{orange}{vs.} Probabilistic Signals of Reliability}
 Methods such as data coverage (as discussed in \S~\ref{sec:related}) generate a binary signal as the reliability score. In contrast, since the binary signal may not be sufficiently informative about how unreliable a prediction is, our proposed \ru measures, generate a probabilistic output. 
In our fifth question, we asked the participants about their preference for the reliability signal output. Participants almost unanimously (98\%) preferred {\bf a numeric value in the range [0,1], where the closer to zero, the more reliable it is}. Only 2\% favored a binary value to show if the output is reliable or not.

\stitle{Q6. Effectiveness of \ru Measures in Practice}
In our final question, we surveyed the effectiveness of our proposed measures when integrated into real-world working systems. 
More particularly, we displayed the mock interfaces from Figure \ref{fig:high_distrust_mock_interface} to the participants and asked if the ``Prediction Reliability'' section would help them to be more confident about how trustworthy the model predictions are. While 76.5\% of the participants answered with a {\bf positive response attesting to the effectiveness of our proposal}, 13.7\% of the participants responded negatively and 9.8\% didn't observe any noticeable differences. 

\color{orange}
\stitle{Limitations of The Study} A limitation of our study is that
\marginpar{R1O5, R2O5}
its target audience was the potential developers of the system 
% more towards the people who build these systems 
such as data scientists, and it did not include the 
% and less towards the people who will be the 
eventual users of such systems. 
Furthermore, in our study, we tried to compare our design choices with other alternatives including the existing methods. These limitations may have introduced some biases to our results and made them not generalizable to every decision-maker and task. 
As part of our future work plan, we would like to extend the study to a broader audience, to include potential decision-makers.
Moreover, it would be interesting to redesign the study to start with a few decision tasks and then ask the comparison questions, in order to maximize the external validity of the study.
% As a future effort, we plan to repeat our study with a broader participant demographics. Moreover, we aim to redesign our study by starting with a few decision tasks and then asking the comparison questions, in order to maximize the external validity of the study.

\color{black}

